SENSEI: Aligning Video Streaming Quality with Dynamic User Sensitivity

This paper aims to improve video streaming by leveraging a simple observation: users are more sensitive to low quality in certain parts of a video than in others. For instance, rebuffering during key moments of a sports video (e.g., before a goal is scored) is more annoying than rebuffering during normal gameplay. Such dynamic quality sensitivity, however, is rarely captured by current approaches, which predict QoE (quality-of-experience) using one-size-fits-all heuristics that are too simplistic to understand the nuances of video content. Instead of proposing yet another heuristic, we take a different approach: we run a separate crowdsourcing experiment for each video to derive users' quality sensitivity at different parts of the video. Of course, the cost of doing this at scale can be prohibitive, but we show that careful experiment design combined with a suite of pruning techniques can make the cost negligible compared to how much content providers invest in content generation and distribution. Our ability to accurately profile time-varying user sensitivity inspires a new approach: dynamically aligning higher (lower) quality with higher (lower) sensitivity periods. We present a new video streaming system called SENSEI that incorporates dynamic quality sensitivity into existing quality adaptation algorithms. We apply SENSEI to two state-of-the-art adaptation algorithms. SENSEI can take seemingly unusual actions: e.g., lowering bitrate (or initiating a rebuffering event) even when bandwidth is sufficient so that it can maintain a higher bitrate without rebuffering when quality sensitivity becomes higher in the near future. Compared to state-of-the-art approaches, SENSEI improves QoE by 15.1% or achieves the same QoE with 26.8% less bandwidth on average.

==> abr-xu.tex <==
\section{\name ABR logic}
\label{sec:abr}

We first introduce the differences between \name and the canonical ABR frameworks (\ref{sec:abr:formu}).
Then, we describe how to build \name upon the existing ABR algorithm frameworks (\ref{sec:abr:alg}).

\subsection{Enabling new adaptation actions}
\label{sec:abr:formu}

We want the video player to (1) lower current quality in hope to improve quality for the next few chunks if they have higher quality sensitivity; and (2) raise current quality slightly over the sustainable level if quality sensitivity is expected to decrease in the next few chunks.
\jc{all these relies on accurate bandwidth prediction}
Instead of reinventing video players from scratch, \name takes a pragmatic stance to work in the framework of existing players and make following changes to its interfaces. 
% This calls for several changes to existing ABR framework. 
Figure~\ref{fig:abr_framework} contrasts the ABR interface of \name with that of typical player.
\begin{packeditemize}
\item {\em Input:} Other than the current player buffer state (how long the buffered content is), the sizes of next chunks at each bitrate level and history throughput measurements, \name ABR also takes as input the sensitivity weights of the next \fillme chunks.
From these weights, the player could infer which future chunks have relatively higher quality sensitivity.
\name's input has the weights of the future chunks, which helps \name make decisions favor the quality sensitive chunks.
\item {\em Output:} Other than the bitrate selection, \name can add a rebuffering event before any unplayed chunk, while the canonical ABR algorithms invoke a rebuffering event only when the player buffer drains out.
\end{packeditemize}

\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.48\linewidth}
    %     \includegraphics[width=1.0\linewidth]{graphs/current_abr.pdf}
    %     \caption{Canonical ABR framework}
    % \end{subfigure}
    %  \hfill
    % \begin{subfigure}[t]{0.48\linewidth}
    % \includegraphics[width=1.0\linewidth]{graphs/our_abr.pdf}
    %     \caption{Nature1}
    %   \end{subfigure}
    \includegraphics[width=1.0\linewidth]{graphs/abr_contrast.pdf}
    \caption{The comparison of ABR algorithm frameworks.}
    \label{fig:abr_framework}
\end{figure}

\subsection{Refactoring current ABR logic}
\label{sec:abr:alg}

\name can be implemented by doing modifications to the existing ABR algorithms.
We will describe the necessary changes to the rule-based (\eg Puffer \cite{yan2020learning}) and non-rule-based (\eg Pensieve \cite{mao2017neural}) ABR algorithms.


The aim of the rule-based ABR algorithms is to maximize the expected QoE of future $H$ chunks, given the number of look-ahead chunks $H$  and the network throughput prediction.
The rule-based ABR algorithm usually select the bitrate for the chunks based on the explicit network throughput.
We will take Puffer as an example and show how to apply dynamic quality sensitivity.

In Puffer, its network predictor $\hat{T}(K_{i+h}^S)$ outputs a discretized probability distribution of predicted transmission time for chunk $i+h$ with bitrate level $S$.
Given the quality of the last sent chunk $K_{i-1}$, and the current buffer level $B_i$, we $v_i^*(B_i, K_{i-1})$ denote as the maximum expected sum of QoE that can be achieved in the $H$-step lookahead horizon.
Thus, our goal is to choose the bitrate $K_i^S$ and the rebuffering time $T_i$ for chunk $i$.
Then, we can have the iteration as
\begin{align}
\begin{split}
    v_i^*(B_i, K_{i-1}) = \max_{K_i^s, T_i} &\left\{ \sum_{t_i}Pr\left[ \hat{T}(K_{i+w}^S) = t_i \right]\cdot \right.\\ 
& \left. \left( w_iQoE_i\left(K_i^s, T_i, K_{i-1}\right) + v_{i+1}^*\left(B_{i+1}, K_{i}^S\right) \right)\right\},\notag
\end{split}
\end{align}
where $w_iQoE_i\left(K_i^s, T_i, K_{i-1}\right)$ is QoE obtained by chunk $i$ and $Pr\left[ \hat{T}(K_{i+h}^S)\right] = t_i$ probability for the transmission time of $K_i^S$ to be $t_i$.
If $T_i$ is $0$, $B_{i+1}$ can be directly derived from the system dynamics in \cite{yin2015control}.
Otherwise, $B_{i+1}$ is $T_i$ plus the buffer level calcualted by \cite{yin2015control} when assuming $T_i=0$.
We can solve this iteration by dynamic programming if we discretize $B_i$ in to bins.

Unlike the rule-based ABR algorithms, the non-rule-based ABR algorithms are a black box.
Fortunately, the input and the clearly defined in such algorithms, by which we could modify the input and output for applying dynamic quality sensitivity.
We take Pensieve as an example to show how to do the modifications.

Pensieve use a deep reinforcement learning network to decide the bitrate version of the next chunks. 
We modify the following aspects in Pensieve to make it be aware of dynamic quality sensitivity:

\mypara{State} In Pensieve, it takes the past throughput, current buffer level and the sizes of next chunks as the state.
Past throughput and next chunks' sizes are used as an indicator of the downloading time of the different bitrate versions of the next chunks.
The current buffer level can determine how aggressive we can make the bitrate selection for the chunk.
To make Pensieve be aware of dynamic quality sensitivity, we also add weights of the future chunks into the state. 
We will discuss the number of future chunks that we should put into the state.

\mypara{Action} The actions at the state $s_i$ have the bitrate for chunk $i$ as well as the rebuffering time added before playing chunk $i$.
In practice, due to the intractable number of states and actions, we discretize the bitrates and rebuffering time into several levels.

\mypara{Reward} The reward depends on the current state $s_i$ and $a_i$. 
If the selected action is a bitrate level, $w_iQoE_i$ defined in Section~\ref{sec:3} is the reward regarding the selected bitrate. 
If the selected action is adding a rebuffering event with duration $T_i$, the reward of this action is the penalty for this rebuffering event we add, \ie $-w_i\beta P_b(T_i)$.

\mypara{Bitrate and rebuffering time selection}
The trained RL model can tell us the probability distribution of actions given a state, \ie the buffer level, next chunks' sizes, past throughput and the weights of future chunks.
\name needs to obtain \emph{both} bitrate level and rebuffering time , while Pensieve just needs to select a bitrate from that distribution.
\name works in the following way: we first select an action by the probalibity distribution. 
If the chosen action is the bitrate level, the player downloads the selected bitrate version.
If the chosen action is the rebuffering event, \name will tell the player to add this rebuffering event before playing this chunk. Then, we change the current buffer size in the original input state, by adding rebuffering time to current buffer level, and run the RL model again, until we get a bitrate selection from the policy.

% \name chooses the action following the probability distribution from the output of the actor network.
% If the chosen action is the bitrate level, the player downloads the selected bitrate version.
% If the chosen action is the rebuffering event, \name will tell the player to add this rebuffering event before playing this chunk. Then, we change the current buffer size in the original input, by adding rebuffering time to current buffer size, and run the RL model again, until we get a bitrate selection from the policy.

% \name concerns the network throughput in the past as the indicator of the future network throughput, and thus, we have the average throughput and the download time of downloading the past $k$ chunks. 
% To be aware of the degree of user attention, $s_t$ needs to have the weights of chunk $i$ and future $r-i$ chunk.
% For estimating the download time of a chunk's different bitrate version, \name need to know the sizes of the bitrate versions.
% We use $n^i_k$ to represent the size of the chunk $i$ with bitrate level $k$.
% % The past $k$ chunks' bitrate $b_{i-k}, b_{i-k+1},\dots, b_{i-1}$ is an indicator of the future chunks' size in different bitrate.

% \mypara{Action} The actions at the state $s_i$ have the bitrate for chunk $i$ as well as the rebuffering time added before playing chunk $i$.
% Thus, our policy is defined as $\pi: \pi(s_i, a_i)\rightarrow [0,1]$, and $\pi(s_i, a_i)$ is the probability which \name chooses the action $a_i$ at state $s_i$.
% In practice, due to the intractable number of states and actions, we discretize the bitrates and rebuffering time into several levels.

% \mypara{Reward} The reward depends on the current state $s_i$ and $a_i$. 
% If the selected action is a bitrate level, $QoE_i$ defined~\eqref{eq:oldqoe_single} is the reward regarding the selected bitrate. 
% If the selected action is adding a rebuffering event, reward is the penalty for this rebuffering event we add, \ie the second term in~\eqref{eq:oldqoe_single}.

% \mypara{Training} The training of \name's follows the standard procedure of A3C \cite{mnih2016asynchronous}. Describe policy gradient here. Emphasis we use discount factor in the reward $\gamma$ to deal with the accuracy of network prediction.

% \name uses the policy from the trained RL model to make the decision of a chunk's bitrate and rebuffering time. The input is as the state in Figure~\ref{fig:our_state}. 
% \name chooses the action following the probability distribution from the output of the actor network.
% If the chosen action is the bitrate level, the player downloads the selected bitrate version.
% If the chosen action is the rebuffering event, \name will tell the player to add this rebuffering event before playing this chunk. Then, we change the current buffer size in the original input, by adding rebuffering time to current buffer size, and run the RL model again, until we get a bitrate selection from the policy.










% At high-level, our main idea is to intentionally lower the QoE of a chunk with less user attention for favoring the chunk with more user attention within a short future.
% Figure~\ref{fig:abr_framework} shows the framework of \name's ABR algorithm and the conventional ones.
% We highlight the difference between our ABR algorithms and the conventional ABR algorithms:
% \begin{itemize}
%     \item \textbf{Input:} \name's input has the weights of the future chunks, which helps \name make decisions that can allocate the temporal network resources to download those chunks.
%     \item \textbf{Output:} Other than the bitrate selection, \name can add a rebuffering event before playing a chunk even the buffer is not empty, while the conventional ABR algorithms invoke a rebuffering event only when the buffer.
%     \item \textbf{Objective:} \name optimizes the expected QoE given a distribution of future network throughput rather than the QoE under the average predicted network throughput in the conventional ABR algorithms.
% \end{itemize}
% Given a predicted network trace, we can make the optimal decision for each chunk under this trace.
% Then, by the probability of the network traces, we can calculate the expected QoE of the rendered video.
% The details of formulation are in Appendix~\ref{sec:appdix:formu}.


% For a source video, the goal of \name's is to maximize the expected QoE under a distribution of the predicted network prediction.
% Assume the network prediction $C_t$ tells the network throughout at future time slot $t$, and $C_t$ is random variable that follows the distribution given by the network predictor.
% The network prediction series for the future $t_{end}$ time slots can be represented as $C_1, C_2, \dots, C_{t_{end}}$, where $t_{end}$ is the maximal possible ending time of the video downloading session.
% Given a network prediction $c_1, c_2, \dots, c_{t_{end}}$, our problem is formulated as
% % Different from other ABR algorithms, we also need to decide whether to put a rebuffering event before playing a chunk in case of the rebuffering event happening in the future chunk with high attention.
% % Suppose $b_i$ is the bitrate for chunk $i$ and $T_i$ is the rebuffering time (or start-up delay for the first chunk). 
% % When making the decision for chunk $i$'s bitrate $b_i$ and rebuffering time level $T_i$, the objective of \name is to maximize the QoE of the rendered video.  
% % The problem is formulated as:
% % \begin{eqnarray}
% % \min_{\substack{b_1,\dots, b_N \\ T_1, \dots, T_N}}  && \mathbb{E}\left[\sum\nolimits_{i=1}^{N} p_iQoE_i(b_i, T_i, b_{i-1})\right] \label{eq:formu:obj}\\
% % \text{s.t.\ \ } && t_{i+1} = \frac{b_i*L}{C_i} - t_{i} \label{eq:formu:start_time_slot}\\
% %  && C_i = \frac{\int_{t_i}^{t_{i+1}}C(t)dt}{t_{i+1} - t_i} \label{eq:formu:avgspeed} \\
% %  && P(C(t) = X) \textrm{ follows the distribution } \Lambda \\
% %  && t_{i+1} \geq (i-1)L + \sum\nolimits_{j=1}^{i} T_j \label{eq:formu:play_after_download} \\
% %  && B_{i+1} = iL - k_{i+1}L - \left(t_{i+1} - k_{i+1}L - T_{k_{i+1}+1}\right)_+\label{eq:formu:buffer_lim} \\
% %  && k_i = \max\{k | \sum\nolimits_{j=1}^k T_j + kL<t_i\} \label{eq:formu:player_status} \\
% %  && B_i \in \left[0, B_{\textrm{max}}\right], B_0 = 0 \label{eq:formu:general_formu}
% % \end{eqnarray}

% \begin{eqnarray}
% \max_{\substack{b_1,\dots, b_N \\ T_1, \dots, T_N}}  && \sum\nolimits_{i=1}^{N} p_iQoE_i(b_i, T_i, b_{i-1}), \label{eq:formu:obj}\\
% \text{s.t.\ \ } && t_i \geq t_{i-1} + D\left(t_{i-1}, S_{i-1}\left(b_{i-1}\right)\right), \label{eq:order_constraint}\\
% && t_i + D(t_i, S_i(t_i)) \leq \sum\nolimits_{j=1}^{i}T_j + (i-1)L, \label{eq:play_after_download}\\
% && D(t_i, S(b_i)) = \min\{j-t_i | \sum_{k=t_i}^{j} c_k \geq S(b_i)\},  \label{eq:download_time}
% \end{eqnarray}
% where $t_i$ is the starting time slot of downloading video chunk $i$, $S_{i}(b_i)$ is the file size of chunk $i$ with bitrate $b_i$, and $D(t_i, S_{i}(b_i))$ is the download time of chunk $i$ with bitrate $b_i$.
% The constraint~\eqref{eq:order_constraint} makes sure one can start to download a chunk only after its previous chunk completes download, and~\eqref{eq:play_after_download} guarantees a chunk can be played only after it is already downloaded.
% The function $D(\cdot,\cdot)$ is defined in~\eqref{eq:download_time}.
% Denote the maximal QoE when the future network is $Q(c_1, \dots, c_{t_{end}})$ that is the solution to the formulation~\eqref{eq:formu:obj}$\sim$\eqref{eq:download_time}.
% Our goal is to maximize the expected QoE as
% \begin{align}
%     \int_{c_1}\dots\int_{c_{t_{end}}} P(c_1, \dots, c_{t_{end}})Q(c_1, \dots, c_{t_{end}})\label{eq:overall_obj}
% \end{align}
% where $P(c_1, \dots, c_{t_{end}})$ is the probability distribution of the predicted network throughout.

% The formulation in~\eqref{eq:formu:obj}$\sim$\eqref{eq:overall_obj} is an stochastic optimal control problem. 
% Its randomness comes from the future network throughput.
% If the predicted network throughput follows the some distribution, \eg one-dimensional Gaussian random walk, we can solve this formulation with the optimal numerical solution \cite{rosseel2012optimal}.
% However, if the distribution is not explainable and written in a explicit form, it is hard to get the optimal numerical solution.
% For those cases, we design a reinforcement-learning-based algorithm for this case in Section~\ref{sec:abr:alg}.
% where $t_i$ is the starting time of downloading video chunk $i$, $C_i$ is predicted average throughput when \name downloads chunk $i$, $C(t)$ is the downloading speed at time $t$, $L$ is the time length of a video chunk, $B_{i}$ is the buffer size when \name starts to download chunk $i$, and $k_i$ is the number of chunks that have been rendered when \name starts to download chunk $i$.
% In our formulation, we start to download a chunk only after its previous chunk is downloaded \eqref{eq:formu:start_time_slot}, and a chunk can be played only after it is already in the buffer~\eqref{eq:formu:play_after_download}.
% The constraints \eqref{eq:formu:buffer_lim}\eqref{eq:formu:general_formu} ensures the buffer will not be larger than the maximum buffer size $B_{\textrm{max}}$ during the video playback.

% The formulation in~\eqref{eq:formu:obj}$\sim$\eqref{eq:formu:general_formu} is an optimal control problem with stochastic partial differential equation (PDE) constraints \cite{rosseel2012optimal}. 
% Its randomness comes from the future network throughput, because the predicted throughput $C(t)$ might not be a number but a probability distribution of throughput.

% \begin{eqnarray} 
% \label{eq:formulation_ours}
%  &&(place holer, will modify)\\
%   \min_{\mathbf{x}, \mathbf{p}}  &&   \sum\nolimits_{j=1}^{M} \sum\nolimits_{v=1}^{M} x_j^{(v)} p_{j}\label{eq:objectives}  \\  % p_{j}
%  \text{s.t}  &&   \sum\nolimits_{j=1}^{M} \sum\nolimits_{v=1}^{M}  x_{j}^{(v)}  U(j,v)  \ge  \log\left( \cfrac{D_{t}}{N_t} \right ),   \label{mu_dis} \\
%   &&   \sum\nolimits_{j=1}^{M} \sum\nolimits_{v=1}^{M}  x_{j}^{(v)} p_{j}  \le P, \label{mu_p} \\
%   && \sum\nolimits_{j=1}^{M} \sum\nolimits_{v=1}^{M} x_{j}^{(v)}  \le M,  \label{mu_au} \\
%   &&  \sum\nolimits_{v=1}^{M} x_{j}^{(v)} \le 1 \ \textrm{and} \ \sum\nolimits_{j=1}^{M} x_{j}^{(v)} \le 1,  \label{mu_ab}  \\
%   &&  x_{j}^{(v)} \in \{0,1\} \;\;\; \textrm{and} \;\;\;\ p_{j}\geq 0  \label{eq:mu_end}.
% \end{eqnarray}

% \subsection{Algorithm Design}
% \label{sec:abr:alg}

% We use \emph{reinforcement learning} (RL) to solve this QoE optimization problem. 
% Compared with other RL-based ABR algorithm (\eg Pensieve\cite{mao2017neural}), \name needs to know the weights and the sizes of the future chunks for making the decisions.
% The details of the RL-based model are illustrated below.

% % \begin{figure}[!htbp]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{graphs/state.pdf}
% %     \caption{The state defined in \name's RL model.}
% %     \label{fig:our_state}
% % \end{figure}

% \mypara{State} The state that taken by the training is shown as in Figure~\ref{fig:our_state}. 
% \name concerns the network throughput in the past as the indicator of the future network throughput, and thus, we have the average throughput and the download time of downloading the past $k$ chunks. 
% To be aware of the degree of user attention, $s_t$ needs to have the weights of chunk $i$ and future $r-i$ chunk.
% For estimating the download time of a chunk's different bitrate version, \name need to know the sizes of the bitrate versions.
% We use $n^i_k$ to represent the size of the chunk $i$ with bitrate level $k$.
% % The past $k$ chunks' bitrate $b_{i-k}, b_{i-k+1},\dots, b_{i-1}$ is an indicator of the future chunks' size in different bitrate.

% \mypara{Action} The actions at the state $s_i$ have the bitrate for chunk $i$ as well as the rebuffering time added before playing chunk $i$.
% Thus, our policy is defined as $\pi: \pi(s_i, a_i)\rightarrow [0,1]$, and $\pi(s_i, a_i)$ is the probability which \name chooses the action $a_i$ at state $s_i$.
% In practice, due to the intractable number of states and actions, we discretize the bitrates and rebuffering time into several levels.

% \mypara{Reward} The reward depends on the current state $s_i$ and $a_i$. 
% If the selected action is a bitrate level, $QoE_i$ defined~\eqref{eq:oldqoe_single} is the reward regarding the selected bitrate. 
% If the selected action is adding a rebuffering event, reward is the penalty for this rebuffering event we add, \ie the second term in~\eqref{eq:oldqoe_single}.

% \mypara{Training} The training of \name's follows the standard procedure of A3C \cite{mnih2016asynchronous}. Describe policy gradient here. Emphasis we use discount factor in the reward $\gamma$ to deal with the accuracy of network prediction.

% \name uses the policy from the trained RL model to make the decision of a chunk's bitrate and rebuffering time. The input is as the state in Figure~\ref{fig:our_state}. 
% \name chooses the action following the probability distribution from the output of the actor network.
% If the chosen action is the bitrate level, the player downloads the selected bitrate version.
% If the chosen action is the rebuffering event, \name will tell the player to add this rebuffering event before playing this chunk. Then, we change the current buffer size in the original input, by adding rebuffering time to current buffer size, and run the RL model again, until we get a bitrate selection from the policy.


==> discuss.tex <==
\section{Discussion}

\jc{dump all ideas that don't fit any section here:
\begin{itemize}
\item need to mention other attention-driven video work (ROI encoding, Pano, etc)
\item how to deal with live video? maybe future work, but need to mention how our ideas might be used there (\eg using real-time reaction of concurrent sessions to create qoe model on-the-fly and apply it to other users)
\end{itemize}
}

==> eval.tex <==





\tightsection{Evaluation}
\label{sec:eval}


%6.1 Setup
%- video dataset
%- network traces
%- performance metrics
%
%6.2 End-to-end evaluation
%- fig 15: overall qoe gains
%- fig 18: qoe gains vs. cost
%- fig 17: increased bandwidth efficiency
%- fig19: qoe gains by videos (genres)
%- fig 20: qoe gains by network conditions (traces)
%
%6.3 Accuracy and cost of QoE modeling
%- qoe prediction accuracy of ours vs. prior models (scatter plots) fig 21
%- qoe gains vs. qoe prediction accuracy (fig ??)
%- effectiveness of cost-cutting techniques: accuracy vs. various cost cutting knobs (fig 22)
%
%6.4 Microbenchmarking \name ABR
%- qoe gains vs. future chunks (fig 27) (maybe also show using more future chunks comes at a slight cost of slower ABR model?)
%- qoe gains vs. bandwidth variation (fig 24)
%- qoe gains under different base abr (fig 26)
%
%6.6 Understanding the "operating regimes"
%- qoe vs. weight variance (fig 27)
%- breakdown of qoe gains (fig 25)
%
%6.7 Systems overheads
%- player CPU (fig 28)
%- increase of manifest file size

% In this section, we first evaluate the performance of \name that optimizes our QoE model. Then, we compare \name's QoE model in Section~\ref{sec:qoe_model} with the state-of-the-art QoE models. The main results are
The evaluation of \name shows several key findings:
\begin{packeditemize}
    \item Compared to recent proposals, \name can improve QoE by 7.7-52.5\% without using more bandwidth and can save 12.1-50.3\% bandwidth while achieving the same QoE. 
    Note that these improvements are on par with those of recent ABR algorithms that use complex ABR logic.
    \item The performance gains of \name come at a cost of \$31.4 
    % and a 78.3-minute delay 
    for a one-minute long video, which is marginal compared to other investments by content providers.
    \item \name can improve QoE prediction accuracy by 11.8-37.1\% over state-of-the-art QoE models.
    \item \name ABR algorithm consistently outperforms baseline ABR algorithms even in presence of bandwidth fluctuation.
    % \item \name's ABR algorithm provides XXX\% more QoE than the existing ABR algorithm by the cost of XXXX USD per minute for the videos.
    % \item \name's ABR algorithm can provide the same QoE with \fillme-\fillme\% less network throughput.
\end{packeditemize}

\begin{table}[t]
\footnotesize
\begin{tabular}{llll}\hline
\textbf{Name} & \textbf{Genre} & \textbf{Length} & \textbf{Source dataset} \\ \hline\hline 
(a) Basket1 & Sports & 3:40 & LIVE-MOBILE \\ \hline
(b) Soccer1 & Sports & 3:20 & LIVE-NFLIX-II \\ \hline
(c) Basket2 & Sports & 3:40 & YouTube-UGC \\ \hline
(d) Soccer2 & Sports & 3:40 & YouTube-UGC \\ \hline
(e) Discus & Sports & 3:40 & YouTube-UGC \\ \hline
(f) Wrestling & Sports & 3:40 & YouTube-UGC \\ \hline
(g) Motor & Sports & 3:40 & YouTube-UGC \\ \hline
(h) Tank & Gaming & 3:40 & YouTube-UGC \\\hline 
(i) FPS1 & Gaming & 3:40 & YouTube-UGC \\\hline
(j) FPS2 & Gaming & 3:40 & YouTube-UGC \\\hline
(k) Mountain & Nature & 1:24 & LIVE-MOBILE \\\hline
(l) Animal & Nature & 3:40 & YouTube-UGC \\\hline
(m) Space & Nature & 3:40 & YouTube-UGC \\\hline
(o) Girl & Animation & 3:40 & YouTube-UGC \\\hline
(n) Lava & Animation & 3:40 & LIVE-NFLIX-II \\\hline
(p) BigBuckBunny & Animation & 9:56 & WaterlooSQOE-III \\\hline
\end{tabular}
\tightcaption{Summary of video set. (See appendix for screenshots and descriptions.)}
\label{tab:summary}
\end{table}


\tightsubsection{Setup}

% We begin by describing the settings of test videos and network traces in our evaluation.
\mypara{Video set and throughput traces} 
Table~\ref{tab:summary} summarizes the genres, lengths and source datasets of our video set.
The videos are selected from four popular datasets.
LIVE-MOBILE~\cite{ghadiyaram2017subjective}, LIVE-NFLX-II~\cite{bampis2018towards} and WaterlooSQOE-III~\cite{duanmu2016quality} are sometimes used to train QoE models in the literature and we complement these sources with videos from a user-generated dataset (YouTube-UGC \cite{wang2019youtube}).
The videos are randomly selected to cover four video genres.
% (\eg sports videos tend to have fast motions vs. nature videos tend to not). 
% We also include two relatively long videos.
To create an adaptive video streaming setup, we chop videos into 4-second chunks and encode each chunk 
% with H.264/MPEG-4 AVC \cite{wiegand2003overview} 
in the five bitrate levels: $\{300,750,1200,1850,2850\}$Kbps (which correspond to $\{240, 360, 480, 720, 1080\}$p on YouTube).
% To test \name and baselines under realistic network conditions, 
We randomly selected 10 throughput traces from two public dataset FCC~\cite{federal2016raw} and 3G/HSDPA~\cite{riiser2013commute}. 
% create a corpus of networks by synthesizing the real network traces in the public datasets: FCC \cite{federal2016raw} and 3G/HSDPA \cite{riiser2013commute}. 
% We randomly select XXXX traces from each dataset for training our ABR algorithm.
% To test the effectiveness of ABR algorithms, 
We restrict our selection to those whose average throughput is between 0.2Mbps and 6Mbps, so that the ABR algorithms can be effective.
(We train Pensieve with 1000 network traces from \cite{mao2017neural}.)
% our bitrate settings and avoiding the trivial cases where selecting the maximum bitrate for all chunks is optimal, the throughput of the selected traces are all from 0.2Mbps to 6Mbps.

% \jc{Xu, how are these videos selected? other than being randomly picked, any other criteria? genre coverage? long vs short? why from multiple datasets not one? why these datasets? }
% % We use the videos in two open datasets LIVE-NFLX-II \cite{bampis2018towards} and YouTube-UGC \cite{wang2019youtube} for evaluating the QoE model and the ABR algorithm in \name. 
% % We randomly select XXX videos from the two datasets. 
% % The details are in Table~\ref{tab:test_video} to evaluate \name. 
% \xu{The source videos are collected from four popular dataset LIVE-MOBILE-STALL, LIVE-NFLX-II WaterlooSQOE-III, YouTube-UGC. LIVE-MOBILE, LIVE-NFLX-II and WaterlooSQOE-III are widely used to train and evaluate the QoE models, while the videos in YouTube-UGC is generated by real users. We select videos across different genres to cover the characteristics of different kinds of videos. For example, sports have many fast motions, nature videos are almost static to show the background, and the objects in gaming/animation videos are moving in a normal pace. To show \name's ability of generalization, we also select 2 long videos (1:24, 9:56).}

% To create an adaptive video streaming setup, 
% In the DASH player, the buffer capacity is 2GB as the default value in Chrome browser. 
% by setting the flags $\texttt{media.cache\_readahead\_limit}$ and $\texttt{media.cache\_resume\_threshold}$ in Firefox or \texttt{--media-cache-size} in Chrome.




% Although many videos only have a handful (5-7) of chunks (each being 4 seconds), we ensure the player must adapt the bandwidth changes 
% make the player start playing right after the first chunk arrives and 
% use a short start-up delay to ensure that the player is always 

\mypara{Baselines}
We compare \name with the following ABR algorithms.
Buffer-based adaptation (BBA)~\cite{huang2014buffer}, Fugu~\cite{yan2020learning}, Pensieve~\cite{mao2017neural}. 
We keep their default settings (\eg same DNN architecture and throughput prediction, etc).
For fairness, we use KSQI as the QoE model for Pensieve, Fugu, and the base QoE model of the \name-modified variations.
This change strictly improves the quality of Pensieve and Fugu, because the QoE models used in their original work are special cases of KSQI.
% \begin{packeditemize}
%     \item Buffer-based adaptation (BBA)~\cite{huang2014buffer} maintains the size of buffer above a threshold and we use the same setting of the original publication: it keeps buffer size above 5 seconds while selects the highest bitrate when buffer size exceeds 15 seconds.
%     % as \cite{huang2014buffer}, \ie, keeping the buffer size is larger than 5 seconds, and the buffer size is larger than 15 seconds, the maximal bitrate is selected automatically.
%     \item Fugu~\cite{yan2020learning} uses current buffer occupancy and throughput prediction for next $h=4$ and picks bitrates that maximize the expected QoE for next $h$ chunks.
%     We keep the throughput predictor of the original paper.
%     % of the chunks in a future window. 
%     % \item MPC \cite{yin2015control}: It 
%     % It predicts the future throughput as the harmonic mean of the experienced throughput of the past XX chunk downloads.
%     \item Pensieve \cite{mao2017neural} selects next chunk's bitrate by feeding current states (past $n$ throughput, buffer occupancy, and chunk sizes) through a RL-trained deep neural net. 
%     We keep its original setting of $n=8$ and the DNN architecture (A3C \cite{mnih2016asynchronous}).
%     % by a probability distribution calculated from a reinforcement-learning-based model that takes the buffer occupancy and past throughput as the input and output the probability of choosing each bitrate level.
% \end{packeditemize}
% By default, 
We use \name-Pensieve as \name, but we confirm that the improvements by \name-Fugu are on par  with \name-Pensieve (Figure~\ref{fig:base-abr}).



\mypara{Performance metrics}
We compare ABR algorithms in three metrics.
% \begin{packeditemize}
% \item 
% {\em QoE (and QoE gain):} 
We evaluate their QoE (normalized to [0,1]) under the same throughput trace and source video and report {\bf QoE gain} of one ABR algorithm ($\QoE_1$) over another ($\QoE_2$), \ie $(\QoE_1-\QoE_2)/\QoE_2$.
% \item 
% {\em Bandwidth saving:} 
We scale down a given throughput trace by different rate and given a target QoE, calculate the {\bf bandwidth savings} by comparing the minimum throughput under which each ABR algorithm achieves the target QoE.
% \item 
% {\em Crowdsourcing cost:} 
We measure {\bf crowdsourcing cost} paid to MTurk to get enough ratings to profile a 1-minute video. Other than \name, this cost is zero.
% \end{packeditemize}



% \jc{mention KSQI as the qoe model for all baselines}



\tightsubsection{End-to-end evaluation}

\mypara{Overall QoE gains}
Figure~\ref{fig:overall_qoe_trace} shows the distributions of QoE gains of \name, Pensieve, and Fugu over BBA, across all combinations of the 10 network traces and 16 source videos.
% We select the traces that are  $\{5, 10, \dots, 95\}$-th percentile of the average throughput from FCC and 3G/HSDPA as the test traces in our evaluation, and they do not have overlap with training traces.
% First, we show the average QoE of the ABR algorithms for different videos under the test cases in Figure~\ref{fig:overall_performance_videos}.
It shows that compared to BBA, \name has at least 14.4\% QoE gains for half of the trace-video combinations, whereas Pensieve's and Fugu's median QoE gains are around 5.7\%.
The tail improvement of \name is greater: \name's QoE gain at 80th percentile is 5.9\%, whereas Pensieve's and Fugu's are 0.1\% and 1.3\% respectively.
% have XXXX\% $\sim$ XXXX\% QoE gain over the existing ABR algorithms across the videos.
% Then, we show the performance of our ABR algorithm under different traces. 
% In Figure~\ref{fig:overall_performance_traces}, we can see \name has XXX\% $\sim$ XXX\% gain over other ABR algorithms under different networks.



\mypara{Bandwidth savings} 
Figure~\ref{fig:overall_performance_qoe_throughput} shows the average QoE of different ABR algorithms across the source videos, under one throughput trace down scaled by different ratio (x-axis). 
(The results are consistent across different throughput traces.)
We see that when setting a target QoE of 0.8, the bandwidth saving of \name is about 27.9\% compared to Pensieve and Fugu and 32.1\% compared to BBA.


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.31\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/trace_video_cdf_qoe.pdf}
         \caption{Distribution of QoE gains over BBA}
         \label{fig:overall_qoe_trace}
       \end{subfigure}
       \hfill
         \begin{subfigure}[t]{0.30\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/qoe_throughput.pdf}
         \caption{QoE vs. bandwidth usage}
         \label{fig:overall_performance_qoe_throughput}
       \end{subfigure}
       \hfill
         \begin{subfigure}[t]{0.31\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/cost_qoe_overall.pdf}
         \caption{Crowdsourcing cost vs. QoE}
         \label{fig:qoe_cost_overall}
       \end{subfigure}
    \tightcaption{End-to-end performance of \name, compared with three baselines, across all videos.
    }
    \label{fig:e2e}
\end{figure*}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{eval_graphs/trace_video_cdf_qoe.pdf}
%     \tightcaption{QoE gains of \name, Pensieve, and Fugu over BBA, across all combinations of traces and source videos.}
%     \label{fig:overall_qoe_trace}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{eval_graphs/qoe_throughput.pdf}
%     \tightcaption{QoE vs. network throughput}
%     \label{fig:overall_performance_qoe_throughput}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{eval_graphs/cost_qoe_overall.pdf}
%     \tightcaption{\name (with and without cost pruning) vs. Pensieve along crowdsourcing cost and resulting QoE. Error bars show standard deviation of the mean. \jc{KSQI => Base ABR!}
%     % \jc{can we add a graph to with delay as the x-axis as well? change legend KSQI to Pensieve (w/ KSQI), change green to black. green is hard to see}
%     }
%     \label{fig:qoe_cost_overall}
% \end{figure}


\mypara{QoE vs. crowdsourcing cost}
\name's QoE gains and bandwidth savings come at a cost.
Figure~\ref{fig:qoe_cost_overall} compares \name (with and without the cost-pruning optimization, which is evaluated separately in Figure~\ref{fig:cost_accuracy}) with Pensieve in terms of their crowdsourcing cost and resulting QoE.
% the budget's impact on performance of \name's ABR algorithm.
% The difference between \name with pruning and without pruning is $3.2\%$.
We see that cost can be pruned by 96.7\% with only 3.1\% degradation in QoE, and \name is still 14.7\% better on average than its base ABR logic (Pensieve with KSQI).
% We see that with XXX USD more budget, we can enumerate XXXX more bitrate or rebuffering time levels.
% We can see that, the QoE improves marginally after we enumerate XXXX bitrate and rebuffereing time levels.
This cost ($\sim$\$31 per 1-minute video) is negligible compared to other expenses incurred by content providers (see discussion in \S\ref{sec:overview}).
% To put \name's crowdsourcing cost (\$31 per 1-minute video) into perspective, Netflix paid \cite{nflxlicense} \$15.3 billion for movie and TV show Licensing, while YouTube paid more than \$170 million to the top 10 YouTube stars \cite{youtubestar}.

% \fillme \jc{how much is it for netflix to get the copyright? how much youtube needs to pay for a popular video uploader? how much is it to buy rent the servers to host 1GB data?}




\mypara{Improvements by videos and traces}
Figure~\ref{fig:overall_performance_videos} shows the QoE gains by videos.
Each bar shows the average QoE gain on the same video across all throughput traces.
We can see there is a significant variance in QoE gains across videos even within the same genre.
So the dynamic quality sensitivity of a video is hardly determined by its content genre. 
Figure~\ref{fig:overall_performance_traces} shows QoE gains by network traces.
Each bar shows the average QoE gain on the same trace across all videos.
Overall, \name has more improvement when average throughput is lower (towards the left). 
It confirms our intuition that, by leveraging dynamic quality sensitivity, \name is better at maintaining a high QoE even when network is under stress.
% \jc{replot the graph first}

% \jc{replot the graph first}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.33\textwidth]{eval_graphs/qoe_gain_by_video.pdf}
    \tightcaption{QoE gains by source videos grouped by genre. }
    \label{fig:overall_performance_videos}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.33\textwidth]{eval_graphs/qoe_gain_by_trace.pdf}
    \tightcaption{\name vs other ABR algorithms by throughput traces (in ascending order of their average throughput)}
    \label{fig:overall_performance_traces}
\end{figure}

% \mypara{Improvements by network conditions}






\mypara{Implications} 
Video streaming literature has been largely focused on developing new ABR algorithms (BBA vs. Pensieve vs. Fugu).
However, the fact that \name's gains over Pensieve (its base ABR logic) are similar to Pensieve's gains over BBA suggests an untapped potential by making an existing ABR algorithm aware of the dynamic quality sensitivity!


\tightsubsection{Microbenchmarking \name QoE model}
Next, we microbenchmark \name's QoE modeling (\S\ref{sec:qoe_model}). 
% and compare its accuracy with state-of-the-art QoE models.
% \mypara{Methodology}
For each source video in our dataset, we divide it into multiple 4-second chunks, and randomly select a chunk's bitrate from $\{$300, 750, 1200, 1850, 2850$\}$Kbps and rebuffering time (or start-up delay for the first chunk) from $[$0, 3$]$ seconds.
We get the ground truth QoE by MTurk surveys (\S\ref{sec:qoe_model:crowd}).
% in a score range of $[$XXX, XXX$]$, and the mean opinion scores of the video sequences are regarded as the ground-truth.
We compare \name QoE model with KSQI~\cite{duanmu2019knowledge}, LSTM-QoE~\cite{eswara2019streaming} and P.1203~\cite{robitza2017modular} (introduced in \S\ref{sec:moti:modelling}).
We randomly split these 640 rendered videos into a train set (400) and a test set (240), which are used to train and test all these QoE models. 
% and train/test these models using the same train/test set.
% We measure QoE prediction accuracy by .

% \mypara{Objective QoE models}
% We choose XXX popular QoE models as the benchmarks:
% \begin{itemize}
%     \item Yin2015 \cite{yin2015control}: It is a linear weighted sum of  bitrate, rebuffering time and bitrate change between adjacent chunks.
%     \item P.1203 \cite{recommendation20171203}: It uses a random forest model to regress the impact of bitrate, rebuffering time and bitrate change based on the users ratings to the video sequences. 
%     \item KSQI \cite{duanmu2019knowledge}: It uses prior knowledge to model the impact of bitrate, rebuffering time and bitrate change. 
%     Using prior knowledge, the QoE of a chunk is a convex function of the QoE factors and the bitrate utility of its previous chunk. 
%     The QoE of a video sequence, it is defined as the sum of the QoE of all the chunks.
% \end{itemize}

\mypara{QoE prediction accuracy}
Figure~\ref{fig:model_accurate} compares the QoE scores estimated by the our QoE model with the baselines. 
Each dot is a generated rendered video.
%and when the prediction is perfect, the dots should line up along a monotonic line in the diagonal direction.
% We recruit real users to rate the video sequences in a score range of $[$XXX, XXX$]$, and the mean opinion scores of the video sequences are regarded as the ground-truth.
% The video sequences are constructed from by by randomly degrading the bitrate or adding a rebuffereing buffer events for the randomly selected chunks.
%  Since the scores estimated by the different QoE models are not aligned in the same range, we are not able to directly calculate the their offsets to the ground-truth.
% Thus, we adopt three statistical criteria to compare our QoE model with the benchmarks: (1) Pearson linear correlation coefficient (PLCC) for the accuracy; (2) Spearman ranking-order correlation (SRCC) and Kendall rank correlation coefficient (KRCC) for the monotonicity.
% The comparison results are in Figure~\ref{fig:model_accurate}. 
% We can see that our QoE model is XXXX\% better in PLCC, XXXX in SRCC, and XXXX in KRCC. 
% \jc{where is KRCC in the graphs?}
We can see that \name's QoE model is visually more concentrated along a diagonal direction than any of the baselines.
We summarize the prediction accuracy in Pearson's Coefficient (PLCC) and the rank correlation in Spearman's Coefficient (SRCC):
On average, \name is over 0.85 in PLCC and 0.84 in SRCC, whereas the baselines are below 0.76 in PLCC and 0.73 in SRCC.

% whereas the baselines are all less than 0.76.
% It also shows the prediction monotonicity by Spearman's Rank Correlation Coefficient (SRCC): \name is 0.84, and the others are less than 0.73.

\begin{figure}[t]
      \begin{subfigure}[t]{0.27\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/our_scores_plot.pdf}
         \caption{\name}
       \end{subfigure}
       \hfill
       \begin{subfigure}[t]{0.23\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/ksqi_scores_plot.pdf}
        \caption{KSQI}
       \end{subfigure}
        \begin{subfigure}[t]{0.225\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/lstm_scores_plot.pdf}
            \caption{\hspace{-0.1cm}LSTM-QoE}
       \end{subfigure}
       \hfill
       \begin{subfigure}[t]{0.225\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/p1203_scores_plot.pdf}
            \caption{P.1203}
       \end{subfigure}
    \tightcaption{QoE prediction accuracy of \name and baseline QoE models}
    \label{fig:model_accurate}
\end{figure}


\mypara{MTurk cost pruning}
Figure~\ref{fig:cost_accuracy} evaluates MTurk cost pruning and its impact on QoE prediction accuracy (PLCC).
We examine four parameters (introduced in \S\ref{sec:qoe_model:scheduling}): the number of bitrate levels ($\NumBitrates$) and the number of rebuffereing lengths ($\NumBufferings$) that can be added in a rendered video, number of ratings per rendered video in two steps ($\NumTurkers = \NumTurkers_1+\NumTurkers_2$), and the difference threshold $\ThreshDiff$ used to pick the chunks to investigate in the second step.
% With more budget, we can enumerate more bitrate and rebuffering time levels for generating the video sequences, which indicates we can have more user ratings to train the QoE model.
% The cost is proportional to the total time of video sequences watched by the participants.
% In our experiment, each video sequence is rated by XX Amazon MTurkers.
% By varying one of these parameters at a time, 
By lowering each parameter from its highest value, we can greatly reduce the cost while imposing less than 3\% drop in accuracy: 
reducing the number of bitrates ($\NumBitrates$ from 5 to 3), the number of rebuffering times ($\NumBufferings$ from 5 to 2), the number of ratings per video (from $\NumTurkers$ from 30 to 10), or raise the difference threshold ($\ThreshDiff$ from 0\% to 6\%).
So the MTurk cost could be saved by setting parameters at their ``sweet spot'' between cost savings and QoE prediction accuracy.
% \jc{link it back to figure~\ref{fig:qoe_cost_overall}}

% First, we evaluate the cost of our QoE model without the cost-saving algorithm in Section~\ref{sec:qoe_model}.

% We then evaluate the cost-saving algorithm in Section~\ref{sec:qoe_model:alg}. 

% From Figures~\ref{fig:cost_accuracy} and~\ref{fig:cost_saving}, we can see that, to achieve the same performance, our cost-saving algorithm can save XXX\% budget to get the same performance, \ie PLCC, SRCC, KRCC.
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.23\textwidth}
    % \centering
    %      \includegraphics[width=1.0\linewidth]{eval_graphs/fewer_bitrate_level_accuracy_plcc.pdf}
    %      \caption{\# of bitrate level}
    %   \end{subfigure}
    %      \begin{subfigure}[t]{0.23\textwidth}
    %          \centering

    %      \includegraphics[width=1.0\linewidth]{eval_graphs/fewer_rebuf_level_plcc.pdf}
    %      \caption{\# of rebuffering time level}
    %   \end{subfigure}
    %       \begin{subfigure}[t]{0.23\textwidth}
    %           \centering
    %      \includegraphics[width=1.0\linewidth]{eval_graphs/fewer_truker_accuracy_plcc.pdf}
    %      \caption{Raters per test video}
    %   \end{subfigure}
    %       \begin{subfigure}[t]{0.23\textwidth}
    %           \centering

    %      \includegraphics[width=1.0\linewidth]{eval_graphs/fewer_chunk_plcc.pdf}
    %      \caption{Filtering threshold}
    %   \end{subfigure}
    \includegraphics[width = 0.43\textwidth]{eval_graphs/cost_eval.pdf}
    \tightcaption{QoE model accuracy changes with costs 
    % \jc{change all x-axis to normalized cost (with the most costly config having 1.) and put the parameter value next to each dot in the graphs}
    }
    \label{fig:cost_accuracy}
\end{figure}

% \mypara{Prediction accuracy on QoE gains}
% Figure~\ref{fig:qoe-vs-accuracy}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{eval_graphs/model_accuracy_qoe.pdf}
%     \caption{QoE vs QoE model accuracy  \xu{from now on all results are simulated}}
%     \label{fig:qoe-vs-accuracy}
% \end{figure}




\tightsubsection{Microbenchmarking \name ABR logic}

Next, we microbenchmark \name ABR logic (\S\ref{sec:abr}).
% and what migh acompare how various factors can affect the effectiveness of ABR.
To scale the experiment out, this part uses real videos and throughput traces but uses QoE predicted by \name to evaluation QoE. This change yields same QoE estimation on average with real user ratings under the same setting (see Figure~\ref{fig:base-abr}).
% With a high QoE prediction accuracy, \name's QoE model shows almost same overall QoE estimation as the MTurk ratings (see Figure~\ref{fig:base-abr}).


\mypara{Impact of bandwidth variance}
Figure~\ref{fig:bw-var} shows the performance of \name under various throughput variance.
We pick one throughput trace and increase its throughput variation by adding a Gaussian noise to control the throughput variance. 
We confirm the results are similar for other throughput traces.
The graph starts from the variance of the original throughput trace. 
With higher variance, \name's QoE degrades, but it still maintains a remarkable gain over its base ABR logic. 
% Even though both \name and the baselines are adversely affected by low throughput prediction accuracy, 
\name is robust because it relies on the ability to predict how likely low quality would occur to {\em only} high quality-sensitivity chunks, rather than all future chunks. 
So as long as the average throughput between now and the next high quality-sensitivity chunk is stable, \name will work well.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.23\textwidth]{eval_graphs/fault_tor_pensieve.pdf}        \includegraphics[width=0.23\textwidth]{eval_graphs/fault_tor_puffer.pdf}

    \tightcaption{QoE under increasing bandwidth variance. 
    % \jc{please show pensieve-based result and Fugu-based result in two separate graphs, change x-axis to standard deviation of throughput.}
    }
    \label{fig:bw-var}
\end{figure}


\mypara{Understanding \name improvements}
Figure~\ref{fig:base-abr} shows that \name achieves comparable improvement when Pensieve and Fugu are the base ABR logic. 
This suggests that \name's effectivenes does not depend on the design of base ABR logic.
Figure~\ref{fig:breakdown} separates the two sources of \name improvements: (1) making the QoE objective aware of dynamic quality sensitivity (\ie the gap between the 1$^{\textrm{st}}$ and 2$^{\textrm{nd}}$ bars), and (2) additional new adaptation actions (initiating rebuffering proactively) 
% to further exploit dynamic quality sensitivity 
(\ie the gap between the 2$^{\textrm{nd}}$ and 3$^{\textrm{rd}}$ bars).
We see that both improves QoE but changing the QoE objective has a greater contribution. 
So even if a content provider cannot control rebuffering, it can still benefit significantly from \name by changing the ABR logic.

% the QoE gains of \name when Pensieve and Fugu are used as its base ABR.
% The QoE gains thus result from changing the QoE objective to be aware of dynamic quality sensitivity and adding the new adaptation actions (whose effects are evaluated separately in Figure~\ref{fig:breakdown}).
% We see that these two optimizations are similarly effectively for these two baselines.
% \jc{insight why Fugu sees less gains?}


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
         \includegraphics[width=0.95\linewidth]{eval_graphs/using_our_model.pdf}
         \caption{Impact of base ABR logic}
         \label{fig:base-abr}
       \end{subfigure}
       \hfill
         \begin{subfigure}[t]{0.48\linewidth}
         \includegraphics[width=1.0\linewidth]{eval_graphs/our_feature.pdf}
         \caption{\name QoE breakdown}
         \label{fig:breakdown}
       \end{subfigure}
    \tightcaption{Understanding \name improvements 
    % \jc{change all x-axis to normalized cost (with the most costly config having 1.) and put the parameter value next to each dot in the graphs}
    }
    \label{fig:understanding}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{eval_graphs/using_our_model.pdf}
%     \tightcaption{Effectiveness of \name optimization over different base ABR algorithms. }
%     \label{fig:base-abr}
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{eval_graphs/our_feature.pdf}
%     \tightcaption{The QoE impact of \name's features}
%     \label{fig:breakdown}
% \end{figure}

% \mypara{Impact of lookahead horizon}
% An important parameter in \name-Pensieve ABR is {\em lookahead horizon}---the number of future chunks whose quality sensitivity weights will be revealed to the ABR. (This has little effect when the base ABR has a fixed lookahead horizon, such as Fugu.)
% A longer horizon in theory allows \name to better improve quality for future high quality-sensitivity chunks by leveraging more low quality-sensitivity chunks, but in practice, it will be constraint by how many future chunks whose throughput can be reliably predicted. 
% We empirically observe that the QoE gains flatten when the lookahead horizon is over 4 chunks.

% In theory, we can reveal all of them and if trained with enough data, Pensieve should figure out
% Figure~\ref{fig:eval_future} examines an important
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{eval_graphs/future_chunks.pdf}
%     \caption{QoE varies with the number of future chunks we look at $k$.}
%     \label{fig:eval_future}
% \end{figure}


% \myparaq{What's the ideal quality sensitivity variance}
% Figure~\ref{fig:regime}
% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.3\textwidth]{eval_graphs/weigt_qoe_gain.pdf}
    
%     \includegraphics[width=0.3\textwidth]{eval_graphs/weigt_qoe_gain_2.pdf}
%     \caption{QoE varies with the variance of the chunk weights.\jc{draw it with more data points}}
%     \label{fig:regime}
% \end{figure}
% \mypara{Improvement breakdown}




\mypara{Systems overhead}
% In runtime, \name imposes negligible overhead in CPU and RAM on the client as its changes are on the input and output of the ABR algorithm. 
We empirically confirm that compared a video player without \name, the runtime overhead of \name is less than 1\% in both CPU cycles and RAM usage.

% \jc{xu, please confirm}


% Table~\ref{tab:system_overhead}
% \begin{table}[t]
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%          CPU &  0.9\% \\
%     \hline
%          Memory & 92.7MB\\
%     \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:system_overhead}
% \end{table}



% \subsection{Understanding \name improvement}























% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{graphs/place_holder.pdf}
%     \caption{System overhead.}
%     \label{fig:my_figure}
% \end{figure}




% \begin{figure*}
%     \centering
%     \includegraphics[width=0.22\textwidth]{eval_graphs/fewer_bitrate_level.pdf}
%     \includegraphics[width=0.22\textwidth]{eval_graphs/fewer_rebuf_level.pdf}
%     \includegraphics[width=0.22\textwidth]{eval_graphs/fewer_truker.pdf}
%     \includegraphics[width=0.22\textwidth]{eval_graphs/save_cost.pdf}    
%     \caption{Cost vs QoE}
%     \label{fig:overall_performance_cost}
% \end{figure*}

% \mypara{QoE vs Throughput}
% Figure~\ref{fig:overall_performance_qoe_throughput} shows the average QoE changes with the throughput.



% \mypara{Looking-ahead horizon}
% How many future chunks we need to look at.



% \mypara{Variability of the weights of chunks} 
% For what kinds of video, we have performance gain.



% \mypara{System overhead}
% Action space vs. performance vs. how large file we need to download

% \subsection{QoE model}





==> intro-deprecated.tex <==
\section{Introduction}

% \item video streaming is (still) important and resource struggles to catch up with video popularity
Ensuring high quality for Internet video streaming is a perennial quest, driven by the ever increasing user expectation for quality of experience (QoE) and the proliferation of larger screen devices and higher resolution videos.
There has been tremendous effort towards striking a better balance between objective quality metrics (low buffering rate, high bitrate, less bitrate switches, etc) and bandwidth demand (\eg~\cite{??,??,??,??}) as well as more accurate QoE models to capture the relationship between user-perceived QoE and objective video quality metrics (\eg~\cite{??,??,??,??}).

% \item conventional wisdom is to build a qoe model that applies to all videos => implicit assumption: people's perception of quality can be decoupled from video content
While a wide range of techniques have been explored, there is a traditional belief that a single desirable QoE model (QoE as a function of objective video quality metrics) should be applicable to different videos and different segments of the same video.
This idea has a pragmatic advantage: it decouples user's perception of video quality from the substance of the video content, so once the video content is encoded into bits, the streaming protocol needs only to focus on optimizing the same quality metrics while adapting to network conditions.

% \item this is not true! examples
Although appealing from a system perspective, this traditional belief is arguably too simplistic.
In live sports videos, for instance, a buffering stall that coincides with point scoring tends to inflict more negatively impact on user experience than buffering stalls elsewhere in the video do.
Intuitively, during {\em critical segments}---video segments (each of a few seconds) that attract more user attention---low quality incidents (buffering stalls, low bitrate, or bitrate switches, etc) are more noticing.
\footnote{Note that some existing QoE models may appear content-dependent too (\eg PSNR~\cite{??,??}(Minerva), SSIM~\cite{??}, VMAF~\cite{??}, \jc{the paper that said buffering at more dynamic scenes are more damaging?}), but they merely considered video frames as matrices of pixels, which hardly translates to how attentive users are to the substance of the content in the whole video.
\jc{maybe mention ROI encoding here if enough space.}}
As the substance of the video content vary in a video and given the limited attention span per viewer, the sensitivity of user-perceived QoE (subjective) to quality metrics can be highly dynamic and unevenly distributed, with several intermittent critical segments where QoE is particularly sensitive to low quality incidents. 

% our insight: leveraging the time-varying qoe sensitivity can have huge benefits.
This paper presents {\em \name}, an adaptive video streaming system that embraces time-varying QoE sensitivity of users to improve user-perceived QoE without using more bandwidth.
For instance, if a critical segment is in the next few seconds and the throughput projection is insufficient to maintain good quality any more, \name will deliberately lower the current quality (\eg adding a short buffering stall or slightly reduce the bitrate) in the hope of ensuring high quality when the key moment segment starts.
Similarly, if a less critical segment is in the near future, \name will increase the quality for the current more critical segment.


% challenges: 1. too costly; 2. today's abr isn't ready (myopic scheduling and no control over buffering, etc)
Of course, the improved QoE-bandwidth tradeoff does not come without a cost. 
First, \name's gains essentially stem from a more {\em granular} approach to QoE modeling---in theory, a separate QoE model is needed per video segment, which can easily become a prohibitive efforts (both in labor and costs).
Second, existing adaptive-bitrate (ABR) algorithms are designed only to handle bandwidth fluctuation and are thus agnostic to the content-dependent variability of QoE models.


\name makes two technical contributions to address these challenges. 

\mypara{Scaling out fine-grained QoE modeling}
First, \name uses crowdsourcing platforms (\eg Amazon MTurk) to automate the process of profiling the QoE sensitivity per video segment. 
Compared to in-lab surveys used widely in QoE literature (\eg~\cite{??,??,??}), crowdsourcing could potentially scale to more videos in an automatic and reproducible manner.
Nonetheless, unlike prior use of crowdsourcing to model QoE per video, modeling QoE per segment would still explode the cost (many videos have at least 10s to 100s of segments).

\name introduces a single weight to each segment that encodes how likely this segment is a critical one and augments existing QoE models by calculating objective quality metrics by re-weighting the per-segment bitrate, buffering stalls, etc.
The rationale behind these per-segment weight is two-fold.
First, these weights are one ``dimensional'', which is significantly easier to profile than profiling the impact of different quality levels (combinations of bitrate, quality switches, buffering stalls, etc).
Second, the QoE model is essentially for different segments, except users pay different attention to them and the heterogeneity in attention is captured by the per-segment weights.
% We are not the first to use crowdsouring in QoE modeling, however, \jc{what's the difference}


\jc{need some back-of-envelope calculation on the cost. also need to explain why vision techniques are inadequate}


\mypara{Refactoring adaptive streaming for dynamic user sensitivity}

%Second, existing adaptive-bitrate (ABR) algorithms adapt only to bandwidth changes and are agnostic to time-varying QoE models. 
%ABR logic cannot be separately from QoE modeling. Can't replace QoE, must change ABR 
%since 

Elaborate our design: 1) Reinforcement learning taking the future chunk's user sensitivity into account; 2) add starting buffer event (video stalling) into the decision base.



Summary of evaluation results.

Summary of our contribution.

Roadmap of the rest paper 

==> intro.tex <==
\section{Introduction}

Importance and trend of video streaming systems.

Introduce what the ABR algorithm is and how ABR algorithm work.

Problems of existing ABR algorithm: (1) they are based on the inaccurate QoE models which have missing parts on the user sensitivity on video quality. Thus, those models will lead to suboptimal decisions; (2) the decisions made by current ABR algorithms only have bitrate detection, NOT have the buffer control in the player.  

{a key insight first before ideas: do bad things in advance}

Our idea 1: make QOE model per video by user study, considering the user sensitivity to the video segments. 

Our idea 2: Add a control logic about buffer event in the video player. We don't have to trigger the buffer event until the buffer is empty. Protect ``sensitive" video chunks

Elaborate our design: 1) Reinforcement learning taking the future chunk's user sensitivity into account; 2) add starting buffer event (video stalling) into the decision base.



Summary of evaluation results.

Summary of our contribution.

Roadmap of the rest paper 

==> motivation-outline.tex <==
\jc{
Xu, please re-organize section 2 with the following flow. 
{\bf make sure each bullet point is one paragraph} (some of your paragraphs are too long...)
some text can be reused though i feel there are quite many missing pieces, so it's better you fix them first and i'll take a pass after that.
\begin{itemize}
\item 2.1: Modeling QoE (Quality of Experience)
\begin{itemize}
    \item why start with qoe modeling: \name is based on a fundamentally different approach to qoe modeling. to understand that, we start with how video qoe is traditionally modeled.
    \item we start with objective metrics on video quality. list popular the metrics, like visual quality, buffering (times, duration, initial buffering, etc), quality smoothness (bitrate switches).
    \item traditionally, the goal of qoe modeling is to predict user satisfaction (user rating or engagement) from objective metrics. introduce three high-level approach: (a) additional model (qoe of each chunk can be independently modeled and ``summed up''); (b) quality incidents can have long-term impact on how user perceive quality on future chunks; (c) use heuristics to capture how pixel values affect the relationship between quality and qoe.
\end{itemize}
\item 2.2 Limitations of current QoE models
\begin{itemize}
    \item we empirically evaluate how accurate they are in predicting qoe. introduce the dataset: a mix of public dataset and our custom dataset? video genre? how you define ground truth? did we average the ratings of multiple users on the same video to avoid cross-user variance (some can be put in appendix)
    \item show the results
    \item Source of the errors: these approaches all strive to predict qoe from objective quality metrics with the assumption that {\em the sequence of objective quality incidents} (need to define quality incident sequence here) captures all that affect QoE. in other words, prior work will predict similar qoe for two videos as long as they have similar quality incident sequences. 
    \item however, these objective quality incidents misses the impact of video content on {\em subjective} attention to quality incidents. we elaborate this effect next.
\end{itemize}
\item 2.3 Temporal variability of user sensitivity
\begin{itemize}
    \item start with a concrete example (the one of the basketball game or soccer game). first, explain we design the experiment this way (how using a single identical rebuffering event keep all prior work to predict the same thing), how you collect data from mturker
    \item explain why buffering has different effects.
    \item generalize it to more examples to demonstrate such temporal variability is prevalent and common across video genres: moments with high tensions in movies, scenic videos (high sensitivity) vs. scenic background (low sensitivity), informative moments (show of score board)
    \item why existing heuristics can't capture them?
\end{itemize}
\item 2.4 Potential QoE gains
\begin{itemize}
    \item so how much qoe gain could modeling use sensitivity more accurately yield? first, explain why there can be gain at all! one reason is that it allows for moving rebuffering to low sensitivity periods. (there can be other ideas, see section 4)
    \item we run a trace-driven simulation to quantify the potential gain from doing just that. explain the methodology.
    \item explain the result
\end{itemize}
\item 2.5 Summary of findings
\end{itemize}
}

==> qoemodel-xu.tex <==
\section{Profiling dynamic quality sensitivity at scale}
\label{sec:qoe_model}


While letting video streaming systems aware of the dynamic quality sensitivity is promising, making it a reality faces two key challenges.
\begin{packedenumerate}
\item {\em How to profile the quality sensitivity of any given video in a scalable and cost-efficient manner (\S\ref{sec:qoe_model})?} 
\item {\em how to design ABR that maximally leverages the temporal variability of quality sensitivity to optimize QoE and save bandwidth (\S\ref{sec:abr})?}
\end{packedenumerate}
%the quality sensitivity for each chunk; and 

To tackle the first challenge, we use two techniques: crowding-sourcing to scale out the profiling of quality sensitivity for any new video (\ref{sec:qoe_model:crowd}) and reweighting video chunks to reduce the cost of identifying (\ref{sec:qoe_model:our_model}).

\subsection{Framework of dynamic quality sensitivity}
\label{sec:qoe_model:our_model}

Our goal is to create a QoE model that does not only depend on the pixel-level induced visual quality and quality incidents but also the dynamic of quality sensitivity, \ie how sensitive the users are to the quality of chunks.
A strawman method built on the prior work is that we train the QoE model based on real user ratings of the video sequences which is an enumeration of all combinations of the quality of the video chunks.
While it is functionally sufficient, the cost can be prohibitive.
For example, for a source video with $10$ chunks, if the numbers of possible bitrate and rebuffering time levels are $5$ and $3$ respectively, we need to collect the ratings of $15^{10}$ video sequences, which is intractable.

We mitigate the cost by two ways: (1) we take a pragmatic stance to build our QoE model direct upon the existing QoE models but reweights each video chunk by a weight that encodes this chunk's quality sensivitiy; (2) we design a crowdsourcing platform that profiles just these per-chunk weights with minimum cost and can easily scale to more videos.

Many existing QoE models, such as KSQI, P.1203, LSTM-QoE, estimate the QoE by weighting the influence of the pixel-level induced visual quality and quality incidents:
\begin{align}
QoE =\sum\nolimits_{i=1}^{1/N} QoE_i(b_i, T_i, b_{i-1}),
\label{eq:oldqoe_overall}
\end{align}
where\footnote{Note that in the existing QoE models, the form could vary significant from an additive to an exponential or logarithmic function.}
\begin{align}
QoE_i(b_i, T_i, b_{i-1}) = &\alpha A(b_i) -\beta P_b(T_i) - \gamma P_s(b_i, b_{i-1}).
\label{eq:oldqoe_single}
\end{align}
We denote $QoE_i$ as the QoE estimation for the a single chunk $i$.
For chunk $i$, $A(b_i)$ is the pixel-level induced visual quality when bitrate is $b_i$, $P_b(T_i)$ represents the penalty of the rebuffering event whose duration is $T_i$, and $P_s(b_i, b_{i-1})$ penalizes the visual quality change from $b_{i-1}$ to $b_{i}$.
The coefficients $\alpha, \beta, \gamma$ weights the influence of each factor in Eq.~\eqref{eq:oldqoe_single}.

Based on the form of the existing models, we can reweight the QoE influence of each chunk as
\begin{align}
QoE &= \sum\nolimits_{i=1}^{1/N} w_iQoE_i(b_i, T_i, b_{i-1}), \label{eq:newqoe_overall}
\end{align}
where $w_i$ is the weight for chunk $i$.
This QoE modeling aligns our insight: \emph{quality sensitivity is largely agnostic to the type of quality incidents.}

Given the form of QoE model, our task is to obtain the weights for the chunks.
We will describe this procedure in Section~\ref{sec:qoe_model:crowd}.  

\begin{figure*}[t]
      \begin{subfigure}[t]{0.22\linewidth}
         \includegraphics[width=1.0\linewidth]{graphs/cv_based_fail.pdf}
         \caption{Sports1}
       \end{subfigure}
       \hfill
       \begin{subfigure}[t]{0.22\linewidth}
         \includegraphics[width=1.0\linewidth]{graphs/cv_based_fail.pdf}
        \caption{Nature1}
       \end{subfigure}
       \hfill
       \begin{subfigure}[t]{0.22\linewidth}
            \includegraphics[width=1.0\linewidth]{graphs/cv_based_fail.pdf}
            \caption{Animation1}
       \end{subfigure}
       \hfill
        \begin{subfigure}[t]{0.22\linewidth}
            \includegraphics[width=1.0\linewidth]{graphs/cv_based_fail.pdf}
            \caption{Gaming1}
       \end{subfigure}
    \caption{Accuracy of user attention estimation by CV-based models \xu{replace the graph with data}}
    \label{fig:cvtech_fail}
\end{figure*}

\subsection{Crowdsourcing at scale}
\label{sec:qoe_model:crowd}

For a source video, our aim is to obtain all the weights of the video chunks in Eq.~\eqref{eq:newqoe_overall}.
We will describe a cost-efficient procedure to profile the dynamic quality sensitivity by using a crowdsourcing platform.

One may argue that we might use some computer-vision (CV) based technique to detect the quality sensitivity .
The related CV techniques could be classified into two categories: video highlight detection and video summarization.
Video highlight detection is to find the chunks that the user will pay more attention than the others.
AMVM \cite{liu2015deriving} argues that the chunks with high motion will be more sensitive to the quality incidents.
It identifies the degree of motion by the motion vectors provided by the H.264 encoder \cite{itu2003264}.
DSN \cite{zhou2018deep} is a deep reinforcement learning model that uses the the dissimilarity between video frames to estimate whether a frame could attract more attention from the users.
The video summarization approaches attempt to extract the chunks which can summarize the whole story of the videos, and the users would pay more attention on those chunks.
Video2GIF \cite{gygli2016video2gif} trains its model by using over 100K user generated video summarizations and their corresponding video sources.

Figure~\ref{fig:cvtech_fail} shows the trend of the quality sensitivity of the chunks is not aligned with that predicted from CV-based models.
Here, the quality sensitivity of a chunk is calculated by 1 minus the QoE of the video sequence with a 1-second rebuffering event inserted to the front of chunk.

The reasons that those CV-based models cannot get the quality sensitivity are two-fold:
\begin{itemize}
    \item The purposes of the models are not exactly aligned with ours: Those models are trained for finding the chunks that the user would pay more attention, and for each chunk, the degree of user attention is not exactly aligned its sensitivity. 
    Thus, when the model is training, the reward or loss function designed for their own purposes would lead the models to another way.
    \item Training features are not enough: As shown in Section~\ref{sec:moti:prop}, the features that affect the quality sensitivity are different across the videos.
    Thus, the videos in our dataset might not be captured by those training videos.
\end{itemize}

Our idea is to use the real user feedback from a crowdsourcing platform, \eg Amazon MTurk \cite{mturk}, to profile the quality sensitivity of those chunks.
The workflow is shown in Figure~\ref{fig:alg_overview}.
Given a monetary budget and the source video, \name generates the video sequences by changing the bitrate and/or adding rebuffering events to the chunk.
Then we collect the ratings of the generated video sequences from a crowdsourcing platform, and regress the weights of the chunks by those ratings.

In the video sequence generator, \name only customizes the quality of one chunk for getting its quality sensitivity.
We do not have to enumerate all the combinations of quality incidents for the chunks, since our model could be an extension from the existing QoE models, and we do not have to remodel the influence of different chunks.
Given a budget and the number of raters we hire on the crowdsourcing platform, we can directly calculate the maximal number of video sequences that we can collect their ratings.
Algorithm~\ref{alg:video_gen} shows the procedure of generating the video sequences.

We can further reduce the cost in the following ways
\begin{itemize}
    \item \textbf{Enumerating fewer quality levels:} Since we are not modeling the QoE impact by different types of quality incidents, it is not necessary to enumerate all the quality levels. 
    We can select a small set of quality levels that can let the chunk stand out against the others.
    \item \textbf{Hiring smaller number of crowd raters to rate a video sequence:}
    Although there is not ground-truth of the QoE for each video sequence, if most raters agree with each other for the QoE of a video sequence, it is not necessary to hire more raters to rate.
    For a video sequence, we can first ask some raters to rate, and if the standard deviation of the ratings collected from the raters, no more works are needed for this video sequences.
    
    \item \textbf{Customizing a smaller number of chunks:} Some video chunks might have similar quality sensitivity.
    Thus, we just need to construct the video sequences from only one of those chunks, and then apply the weight of this chunk to other similar chunks.
    If the raters react similarly to the video sequences that have the same quality incident at two chunks, we could identify the two chunks have similar quality sensitivity.  
\end{itemize}

In the procedure of user rating collection, we show the generated video sequences to the raters one by one.
After watching each video sequence, the raters are required to rate the video sequence they just saw and tell us what type of quality incident they just saw.
We show the interface in Appendix XX.

We need to validate the ratings is meaningful, \ie the crowd raters do not give us random ratings for the video sequences.
Although there is no standard method, in our case, we use the user engagement to validate their ratings.

\mypara{Hard rules} In the beginning of the test, the raters should read the instruction carefully.
In the instruction, we define what they have to do during this survey.
For example, after watching a video sequence, the raters must give their rating and select what quality incidents they just saw, otherwise, the survey cannot go on.

\mypara{Time spend on the survey} The time spent on the survey is a good indicator of whether the worker treat this survey seriously or not.
We monitor the time of the reading the instruction, watching and rating each video sequence.
If a rater spends much less than time than the average or it does not watch the whole video sequence, we identify this rater is likely to give random feedback.

\mypara{Control questions} A popular technique of feedback validation is to check whether the raters give the correct answer to the questions whose answers are already known \cite{hossfeld2013best}.
In our survey, we add two control questions: (1) we ask the raters rate a video sequence without any quality incidents, and this video sequence is supposed to have the highest rating; (2) after watching each video sequences, the raters need to tell us what quality incident they just saw. 

For the long source videos, we are not able to show the video sequences that has the quality incidents only on one chunk, since the QoE impact we could observe might be marginal due to the memory effect.
For those videos, we first show the raters the whole video without any quality incident.
It is for giving them the expectation of the quality of each part in the video.
Then, we can chop the source video into multiple clips in which each of them contains several chunks, and we can generate the video sequences based on those clips, and show them to the crowd raters.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{graphs/alg_overview.pdf}
    \caption{Workflow of profiling dynamic quality sensitivity using crowdsourcing platforms}
    \label{fig:alg_overview}
\end{figure}


% We use \emph{user study} to obtain the weights of video chunks. 
% As shown in Figure~\ref{fig:alg_overview}, given a monetary budget $B$, we can calculate the number of video sequences $N_\mathcal{S}$ we can generate in the user study as $N_{\mathcal{S}} = B/(\text{hourly wage}*N_\text{MTurker}*L)$, where $N_{\text{MTurkers}}$ is the number of the MTurkers we hire in the user study and $L$ is the time length of the source video.
% We need to generate the video sequences whose chunks are with different bitrate and rebuffering time.
% Since we cannot enumerate all possible bitrate and rebuffering time, we have to discretize bitrate and rebuffering time for generating the video sequences.
% Suppose the bitrate and rebuffering time are discretized as $M$ and $K$ respectively.
% Using those parameters, the video sequences are generated by our video sequence generator. Then, the video sequences will be rated by the MTurkers, and we use the ratings to calculate the weights by linear regression \cite{freedman2009statistical}.

% The details of video sequence generator is shown Algorithm~\ref{alg:video_gen}.
% For a video sequence with $N$ chunks, to solve this linear system in~\eqref{eq:newqoe_overall} we need at least $N$ video sequences, and those video sequences should be \emph{linear independent} in terms of those weights.
% In each video sequence generated by the algorithm, only one chunk has different quality with the other chunks that are with the same bitrate level and no rebuffering event.
% That is to directly ask the users about how much QoE impact by this particular chunk.
% % That is to remove the QoE impact from other chunks when we calculate a chunk's weight.
% For each chunk we can have $N_{\mathcal{S}}/N$ video sequences that are with different bitrate levels or rebuffer levels from those of other chunks.
% For constructing the video sequences for chunk $i$, we randomly select chunk $i$'s bitrate $b_i$ and rebuffering time $T_i$ from the uniform distributions $[1\dots M]$ and $[1 \dots K]$ respectively, and we keep the other chunks have the same bitrate $b_o$ and no rebuffering time between those chunks.

\SetKwInOut{Input}{Input}
\begin{algorithm}[!t]
{
    \small
    \DontPrintSemicolon
    \KwIn{(1) Total number of video sequences: $N_{\mathcal{S}}$\\
    \quad\quad\quad (2) bitrate level: $M$\\
    \quad\quad\quad (3) rebuffering time level: $K$\\
    \quad\quad\quad (4) number of chunks : $N$\\
    }
    \KwOut{The video sequences: $\mathcal{S}$\\}
    $\mathcal{S}\leftarrow \emptyset$\\
    \For {$i \leftarrow 1$ \KwTo $N$}{
        $counter \leftarrow 0$\\
        \While {$counter < N_{\mathcal{S}}/N$}{
            \tcc{select chunk $i$'s bitrate}
            $b_i \leftarrow \text{randomly select from}\  \{1\dots M-1$\}\\
            \tcc{select chunk $i$'s rebuffering time}
            $T_i \leftarrow \text{randomly select from}\  \{1\dots K$\}\\
            \tcc{select other chunks' bitrate}
            $b_o \leftarrow M$\\
            $V \leftarrow$ construct the video sequence by $b_o, b_i, T_i$\\            
            \If {$V \notin \mathcal{S} $} {
                $\mathcal{S} \leftarrow \mathcal{S}\cup \{V\}$\\
                $counter \leftarrow counter + 1$\\
            }
        }
    }
    \textbf{return} $\mathcal{S}$
    \caption{Video Sequence Generator}
	\label{alg:video_gen}
}
\end{algorithm}

% We can further save the cost based on an observation: \emph{if two adjacent chunks have similar degree of user attention, they have similar weights.} 
% Thus, we do not have to collect the user ratings of all the video sequences $\mathcal{S}$ generated from Algorithm~\ref{alg:video_gen}. 
% We show the procedure of pruning the video sequences $\mathcal{S}$ in Algorithm~\ref{alg:video_gen_save}.
% First, the MTurkers rate the degree of user attention as in Section~\ref{sec:moti:missing}.
% We conduct a user study in which we ask the MTurkers to vote which chunk they think is important in terms of content.
% A chunk's degree of attention is the votes got from the MTurkers.
% We denote the degree of attention of the chunks $1 \dots N$ as $\mathcal{I}=\{I_1, \dots, I_N\}$.
% Then, if the difference of the degree of user attention between adjacent chunks is smaller than a threshold $\delta$, those adjacent chunks could have the same weight.
% The MTurkers just need to rate $N_{S}/N$ out of all the video sequences where those adjacent chunks are customized.
% We will evaluate how efficiently we build a per-video QoE model in Section~\ref{sec:eval}.
% \begin{algorithm}[!t]
% {
%     \small
%     \DontPrintSemicolon
%     \KwIn{(1) Video sequences: $\mathcal{S}$\\
%     \quad\quad\quad (2) Degree of attention $\mathcal{I}$\\
%     \quad\quad\quad (3) Threshold $\delta$ \\
%     }
%     \KwOut{Pruned video sequences: $\mathcal{S}_{\text{pruned}}$\\}
%     \tcc{Initialization}
%     $\forall i, S_i \leftarrow$ the video sequences that customize chunk $i$ in $\mathcal{S}$ \\
%     $idx \leftarrow 2$\\
%     \While {$idx <= N$} {
%         $idxset \leftarrow \{i\}$ \\
%         \While { ($idx+1 <= N$) \textbf{and} ($|I_{idx+1}-I_{idx}| <\delta$) } {
%             $idxset \leftarrow idxset \cup \{idx+1\}$ \\
%             $idx \leftarrow idx + 1$\\
%         }
%         $S\leftarrow$ randomly select $N_{\mathcal{S}}/N$ video sequences from $\{ \cup S_i| i \in idxset\}$ \\
%         $\forall i\in idxset, S_i\leftarrow$ S\\
%     }
%     $\mathcal{S}_{\text{pruned}} \leftarrow S_1 \cup S_2 \cup \dots \cup S_N$ \\
%     \textbf{return} $\mathcal{S}_{\text{pruned}}$
%     \caption{Pruning video sequences}
% 	\label{alg:video_gen_save}
% }
% \end{algorithm}


==> related-xu.tex <==
\section{Related Work}
\label{sec:relatedwork}
We briefly survey the most related work on video QoE model, ABR algorithm and user study platform.

\mypara{Video QoE modeling}
Recently, QoE modeling for adaptive video streaming has attracted much attention from industry and academia.
Due to the intractable number of the factors that affect QoE, the QoE models can be categorized by their observation space.
The video quality assessment (VQA) models evaluates the pixel-level visual quality of the test videos.
To estimate the visual quality, PSNR \cite{gonzalez2004digital} computes the pixel difference between the source video and the test video, and
SSIM \cite{wang2004image, rehman2015display} and STRRED \cite{soundararajan2012video} use structural information of frames.
Recent VQA models exploit the user feedback in term of ratings to estimate the user-perceived quality.
VMAF \cite{vmaf} uses a support vector machin (SVM) based regression, while DeepVQA \cite{kim2018deep} tries to links the video pixels to user ratings by deep reinforcement learning.
Other than pixel-level visual quality, advanced QoE models also take the quality incidents into account.
Those models weight the QoE influnce of the quality incidents and the visual quality quality by different regression models: nonlinear autoregressive exogenous (NARX) model \cite{bampis2017continuous, bampis2017augmented}, quadratic programming \cite{duanmu2016quality, duanmu2019knowledge}, linear regression \cite{de2013model}, Hammerstein-Wiener model \cite{chen2014modeling}, long short-term memory network \cite{eswara2019streaming} etc.

\mypara{ABR algorithms}
Recent years have witnessed the prevalence of DASH systems where the ABR algorithms is the core part.
Early ABR algorithms can be grouped into buffer-based and rate-based approaches.
The rate-based ABR algorithms \cite{jiang2012improving, li2014probe} try to match the bitrate to the network throughput, while the buffer-based approaches \cite{huang2014buffer,spiteri2016bola,spiteri2019theory} consider the buffer occupancy to decide the bitrate version of the next chunks.
The advanced ABR algorithms take both buffer occupancy and future network throughput into account. MPC \cite{yin2015control} uses a control-theory-based algorithm to optimize the QoE of the chunks in a horizon. CS2P's \cite{sun2016cs2p} uses the MPC's ABR algorithm but a better network predictor that regards the network throughput as discreted states and will notify the systems when the throughput state changes. Puffer uses a machine-learning method to predict throughput as a discrete probability distribution, by which Puffer optimizes the expected QoE of the future chunks by MPC controller.
Pensieve takes the buffer occupancy and the past throughput as the input, and use a deep reinforcement learning model to select the bitrate for the next chunks.
Oboe \cite{akhtar2018oboe} claims that the performance of the ABR algorithms highly depend on the parameters, and Oboe designs an algorithm for finding the best set of the parameters for the existing ABR algorithsm.

\mypara{QoE research using crowdsourcing} Recent research on QoE heavily relies on the subjective evaluation collected from real end users.
The low cost and flexible of crowdsourcing has attracted much attention from  industry and academia.
The crowdsourcing platforms, \eg Amazon MTurk\cite{mturk} and Microworkers\cite{microworkers}, provide the most direct and unfiltered access to the participants, which enables a fast deployment of a large-scale user study.
Upon those platform, a number of frameworks are built for multimedia user study.
WESP \cite{rainer2013web} provides APIs to configure each component of the user study, \eg pre-questionnaire, and control questions.
Its APIs also allows us to design the survey on the common UI, \eg single stimulus, double
stimulus, pair comparison or continuous quality evaluation.
Quadrant of Euphoria (QE) \cite{chen2010quadrant} uses pair comparison instead of a MOS test.
In QE, the QoE of a test multimedia content is estimated by the probability that this content has larger QoE than another random content.
Eyeorg \cite{varvello2016eyeorg} studies relationship between user-perceived web loading time and QoE. Like QE, Eyeorg shows the web page loading event side by side to increase the realibility of the user ratings.
To control the page loading time, Eyeorg shows the videos that record the page loading events with different latency to the raters.
YoutubeQoE \cite{hossfeld2011quantification} is a platform that can collect the user feedback for the videos.
It collects the user ratings (1-5) to quantify the QoE of the test videos.
To ensure the reliability of the user ratings, YouTubeQoE uses the control questions, \eg what content the video is about.

